Unsupervised 3D End-to-End Medical Image Registration with Volume Tweening Network

3D medical image registration is of great clinical importance. However, supervised learning methods require a large amount of accurately annotated corresponding control points (or morphing), which are very difficult to obtain. Unsupervised learning methods ease the burden of manual annotation by exploiting unlabeled data without supervision. In this paper, we propose a new unsupervised learning method using convolutional neural networks under an end-to-end framework, Volume Tweening Network (VTN), for 3D medical image registration. We propose three innovative technical components: (1) An end-to-end cascading scheme that resolves large displacement; (2) An efficient integration of affine registration network; and (3) An additional invertibility loss that encourages backward consistency. Experiments demonstrate that our algorithm is 880x faster (or 3.3x faster without GPU acceleration) than traditional optimization-based methods and achieves state-of-theart performance in medical image registration.

==> app-figs.tex <==
\section{Additional Figures}

This section includes several example illustrations of results.

\subsection{Figures for Liver Registration}

\LiverMethodsFigure{!p}

\figureref{liver-algo-fig} compares the methods listed in \tableref{liver-algo-table} except for ``ADDD'' (which is similar to ``ADDD + inv''), where three landmarks are selected and the sections of the volumes at the height of each landmark \emph{in the fixed image} are rendered. This means the red crosses (landmarks in the moving and warped images) indicate the projections of the landmarks onto those planes. It should be noted that though the sections of the warped segmentations seem to be less overlapping with those of the fixed one, the Segmentation IoU is computed for the volume and not the sections. It might well be the case that the overlap is not so satisfactory when viewed from those planes yet is better when viewed as a volume. Similarly, overlapping red and yellow crosses do not necessarily imply overlapping fixed and warped landmarks as they might deviate along $z$-axis.

\LiverCascadeFigure{!p}

In \figureref{liver-cascade-fig}, we compare ADDD + inv, ADDD, ADD, AD and D, four differently cascaded networks, one with an extra loss term. The data prove cascading networks significantly improves the performance, because it better registers images with large displacement.

\LiverCascadeProgressFigure{!p}

\figureref{liver-cascade-progress-fig} illustrates the intermediate flows produced by ADDD network on two CT liver scans. Each subnetwork registers the images better, increasing Segmentation IoU and lowering Landmark Distance.

\subsection{Figures for Brain Registration}

\BrainMethodsFigure{!p}

\figureref{brain-algo-fig} exemplifies the methods on two brain scans. Comparison between our methods and traditional methods proves the applicability of our methods to 3D brain registration. Comparison between ADD and {DD\xtraAntsAffine} shows that integrating affine registration subnetwork is effective.

\BrainSupFigure{!p}

\figureref{brain-sup-fig} compares unsupervised and supervised {\ModelNameShort}. The figure clearly demonstrates that supervision by the ground-truth generated by traditional methods (ANTs here) does not yield better performance that using our unsupervised training method. Moreover, acquiring the ground-truth is time-consuming, hence not worth the effort.

\BrainCascadeFigure{!p}

In \figureref{brain-cascade-fig}, there are two dimensions of comparison. Comparing ADD and AD, or {D\xtraAntsAffine} and {DD\xtraAntsAffine} shows that performance is gained by cascading more subnetworks. Comparing ADD and {DD\xtraAntsAffine}, or AD and {D\xtraAntsAffine} shows that integrating affine registration into the method yields better registration accuracy.


==> app-impl.tex <==
\section{Notes to Implementation}

\subsection{TensorFlow Custom Operations}

We choose TensorFlow \cite{tensorflow} as our platform. Several operations need to be implemented as custom operations to reduce memory footprint. These include functionalities to warp images, compute moments of random variables, approximate entropy, etc.% Our code is available at \placeholder{repo address}.

\subsection{Warp and Domain Shrinking}

Recall that the domain of a flow is the cuboid $\Omega$ on which the image is defined. Consider the flow $f:\Omega\to\mathbb{R}^3$, define its ``valid domain'' as
\begin{equation}
\ValidDom f=\left\{{\omega\in\Omega:\omega+f(\omega)\in\Omega}\right\},
\end{equation}
i.e., those points that are kept in $\Omega$ when displaced according to the flow. Ideally the valid domain could be the same as $\Omega$. However, sometimes part of the moving image is cropped out in the fixed one, or due to algorithm's imperfectness, the valid domain might unavoidably be a proper subset of $\Omega$, which is called domain shrinking. In our network, an image might need to be warped multiple times. Warping with a domain-shrinking flow field will introduce glitches on the boundaries. This is especially undesirable if the warping is used to compose inverse flows, which makes values on the boundaries non-zero artefacts. To partially resolve the problem, we assume the central part of the composed flow is still valid, hence only compute invertibility loss in the central area.

\subsection{Flow Composition}

If we are composing two dense flows, there is nothing much interesting to do other than following the definition. However, if the first flow to be composed is actually an affine transform, alternative formula for composition could speed up computation, avoid interpolation and eliminate further domain shrinking. Simple calculation gives
\begin{equation}
\left({Ax+b}\right)\star f=\left({I+A}\right)f+Ax+b,
\end{equation}
which does not involve warping at all.

\subsection{Orthogonality Loss}

Computing orthogonality loss involves signular values of $I+A$. The square of these singular values are exactly the eigenvalues of ${\left({I+A}\right)}^\Transpose{\left({I+A}\right)}$. Since the loss is a symmetric fraction of these eigenvalues, it can be rewritten as a fraction of the characteristic polynomial of ${\left({I+A}\right)}^\Transpose{\left({I+A}\right)}$ by Vi{\`e}te's theorem. The formula is cumbersome but not difficult to derive.

\subsection{Command Lines for Traditional Methods}

In this section we record the command lines used for traditional methods.

For registration (liver and brain) with ANTs \cite{avants2009advanced}, the command we use is the following:\\
\texttt{antsRegistration -d 3 -o <OutFileSpec>\\
-u 1 -w [0.025,0.975]\\
-r [<Fixed>,<Moving>,1]\\
-t Rigid[0.1]\\
-m MI[<Fixed>,<Moving>,1,32,Regular,0.2]\\
-c [2000x2000x2000,1e-9,15]\\
-s 2x1x0 -f 4x2x1\\
-t Affine[0.1]\\
-m MI[<Fixed>,<Moving>,1,32,Regular,0.1]\\
-c [2000x2000x2000,1e-9,15]\\
-s 2x1x0 -f 4x2x1\\
-t SyN[0.15,3.0,0.0]\\
-m CC[<Fixed>,<Moving>,1,4]\\
-c [100x100x100x50,1e-9,15]\\
-s 3x2x1x0 -f 6x4x2x1}
% Parameters found in "ants.py", "create_gcr_jobs.py" and "registration_runner.py", search "antsRegistration".

For registration (liver and brain) with Elastix \cite{elastix}, the command we use is the following:\\
\texttt{elastix -f <Fixed> -m <Moving>\\
-out <OutFileSpec>\\
-p Affine -p BSpline{\textunderscore}1000}
% Parameters found in "liver_baseline.ipynb", search "registrate".

For affine pre-alignment (brain) with ANTs, the command we use is the following:\\
\texttt{antsRegistration -d 3 -o <OutFileSpec>\\
-u 1 -w [0.025,0.975]\\
-r [<Atlas>,<Image>,1]\\
-t Rigid[0.1]\\
-m MI[<Atlas>,<Image>,1,32,Regular,0.2]\\
-c [2000x2000x2000,1e-9,15]\\
-s 2x1x0 -f 4x2x1 -t Affine[0.1]\\
-m MI[<Atlas>,<Image>,1,32,Regular,0.1]\\
-c [2000x2000x2000,1e-9,15]\\
-s 2x1x0 -f 4x2x1}


==> app-loss.tex <==
\section{Loss Functions}

This section lists some other loss functions that could be used for training the network.

\subsection{$L_2$ Loss}

$L_2$ loss (or mean square error) measures the difference between intensities of the images at each voxel, it is defined as
\begin{equation}
L_{\MSE}\left({I_1,I_2}\right)=\frac{1}{\left|\Omega\right|}\sum_{x\in\Omega}{{\left({I_1\left(x\right)-I_2\left(x\right)}\right)}^2}.
\end{equation}
$L_2$ loss is straight-forward and easy to implement, but it is not very informative if the fixing and moving images have different imaging parameters. The disadvantage manifests itself especially when the images are inter-subject, or are imaged using devices from different manufacturers.

\subsection{Mutual Information}

Again we will regard the images as random variables. The entropy of a discrete random variable $X$ is
\begin{equation}
H\left(X\right)=-\sum_{x}{p_{_X}\left(x\right)\log{p_{_X}\left(x\right)}},
\end{equation}
and the mutual information of two discrete random variables $X,Y$ is
\begin{equation}
\MutualInfo{X}{Y}=H\left(X\right)+H\left(Y\right)-H\left({X,Y}\right).
\end{equation}
Mutual information of two images measures how much the two variables are related by \emph{some} function. Presumably the intensities of corresponding anatomical structures in the fixed and moving images should be related via \emph{some} function, which might be non-linear. Therefore, mutual information should be more resistant to non-linear intensity variation. Indeed, variants of mutual information have been the gold standard among medical image registration metrics \cite{mi-reg-freeform,Hermosillo2002,overlap-inv-mi,mi-reg-survey}. The downside of this family of loss functions is that adapting them in neural networks is not completely trivial.

From the definition, computing mutual information reduces to computing entropies. Given a series of independent observations $x_1,\dots,x_n$ to a random variable $X$, a na\"ive estimation of $H\left(X\right)$ is
\begin{equation}
\label{naive-entropy-estimation}
H\left(X\right)\approx\frac1n\sum_{i=1}^{n}{\log\frac{\left|\left\{{j:x_j=x_i}\right\}\right|}{n}}.
\end{equation}
Though \equationref{naive-entropy-estimation} systematically underestimates the entropy and various improved algorithms have been developed \cite{mi-entropy-estimation,valiant-entropy}, it is still the simplest estimator. However, there is one obstacle keeping it from being used in neural networks, ``binning.'' Traditionally, binning is required for two reasons: that the metric is more robust against random fluctuations in intensities, which will be effaced by binning; and that directly estimating entropy of continuous random variable from unbinned observations is generally more difficult than the binned, discrete alternative. However, the downside of binning is that the operation makes gradient vanish almost everywhere, effectively making the problem of maximizing mutual information a discrete optimization problem, disqualifying gradient descent and other gradient-based optimizers. To tackle the problem, we rewrite \equationref{naive-entropy-estimation} as
\begin{equation}
H\left(X\right)\approx\frac1n\sum_{i=1}^{n}{\log\frac{\sum_{j=1}^{n}{z\left({x_i-x_j}\right)}}{n}},
\end{equation}
where $z\left(x\right)$ is $1$ if $x=0$, and $0$ otherwise. Now, we are ready to replace $z$ with an approximation, e.g., $z_\lambda(x)=e^{-\lambda\left|x\right|}$ for $\lambda>0$. Furthermore, using this formula boosts the time of computation to the order of number of observations squared. Thus, we need to randomly sample a subset of locations to compute entropy.


==> app-vtn-naming.tex <==
\section{Naming of {\ModelNameLong}}

\VTNNamingFigure{!h}

In \figureref{vtn-naming}, intermediate warped images as well as the fixed and moving images are projected and rendered, giving a straight-forward illustration of how the image is transformed step by step by a cascaded network. This explains the naming {\emphModelNameLong} -- due to the cascaded nature of the network, the intermediate images look like frames in a shape tweening animation from the moving image to the fixed image.

